Anomalous Diffusion of Lithium-Anion Clusters in Ionic Liquids

Lithium-ion transport is significantly retarded in ionic liquids (ILs). In this work, we performed extensive molecular dynamics (MD) simulations to mimic the kinetics of lithium ions in ILs using [\emph{N}-methyl-\emph{N}-propylpyrrolidium (pyr$_{13}$)][bis(trifluoromethanesulfonyl)imide (Ntf$_{2}$)] with added LiNtf$_{2}$ salt. And we analyzed their transport, developing a two-state model and comparing it to the machine learning-identified states. The transport of lithium ions involves local shell exchanges of the Ntf$_{2}$ in the medium. We calculated train size distributions over various time scales. The train size distribution decays as a power law, representing non-Poissonian bursty shell exchanges. We analyzed the non-Poissonian processes of lithium ions transport as a two-state (soft and hard) model. We analytically calculated the transition probability of the two-state model, which fits well to the lifetime autocorrelation functions of LiNtf$_{2}$ shells. To identify two states, we introduced the graph neutral network incorporating local molecular structure. The results reveal that the shell-soft state mainly contributes to the transport of the lithium ions, and their contribution is more important in low temperatures. Hence, it is the key for enhanced lithium ion transport to increase the fraction of the shell-soft state.

==> 55.PDF.tex <==
\subsection{Train Size Distributions by varying $\Delta t$}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{FigS05.png}
    \caption{Train size distributions by varying $\Delta t$; \footnotesize{we varied train size $\Delta t$ (main text),  $\Delta t/2$ (green, $\beta=1.292$), $\Delta t/3$ (blue, $\beta=1.311$), and $\Delta t/4$ (orange, $\beta=1.296$}}
    \label{fig:varying_train_size}
\end{figure}

We calculated train size distributions by varying $\Delta t$ which is defined from an average inter-shell exchange time. As stated in the main text, they show changing $\Delta t$ does not change the power-law exponent.

==> 60.AuthorContri.tex <==
\renewcommand\thesection{}
\section{Author Contribution}
YSJ and WBL designed the project. YSJ and YKL developed the theoretical formula and performed numerical calculations. YKL, JBC, and JSK performed simulations. YSJ, YKL, JBC, and WBL analyzed data and wrote the manuscript.

\section{Data Availability}
The authors will provide data on reasonable request. 

\section{Acknowledgement}
This research was supported by the National Research Foundation of Korea(NRF) grant funded by the Korea government(MSIT) 2018M3D1A1058624, and 2021R1A2C1014562.
